A Two-Stage Stochastic Programming Model for Car-Sharing Problem using Kernel Density Estimation

Car-sharing problem is a popular research field in sharing economy. In this paper, we investigate the car-sharing re-balancing problem under uncertain demands. An innovative framework that integrates a non-parametric approach - kernel density estimation (KDE) and a two-stage stochastic programming (SP) model are proposed. Specifically, the probability distributions are derived from New York taxi trip data sets by KDE, which is used as the input uncertain parameters for SP. Additionally, the car-sharing problem is formulated as a two-stage SP model which aims to maximize the overall profit. Meanwhile, a Monte Carlo method called sample average approximation (SAA) and Benders decomposition algorithm is introduced to solve the large-scale optimization model. Finally, the experimental validations show that the proposed framework outperforms the existing works in terms of outcomes.

==> 2-literature.tex <==

\section{Literature Review}
Generally, the car-sharing problem can be categorized into four types\cite{vosooghi2017critical},\cite{illgen2018literature}, e.g. one-way base-station, one-way free-floating, one-way shared autonomous vehicles and round trip. Most of the work focus on relocation (re-balancing) issue, which plays the most essential role in car-sharing problem. In order to solve the problem, several optimization approaches are under investigation including complicating determinate modeling and optimization under uncertainty. 

\par
For deterministic model, Gambella et al. \cite{gambella2018optimizing} propose an MIP model along with two heuristic algorithms to optimize electric vehicle relocation problem, Huang et al.\cite{huang2018solving} investigate one-way station-based relocation considering non-linear demand, an mixed integer non-linear model is proposed, Xu et al.\cite{xu2018electric} study the electric vehicle fleet size and trip pricing (EVFS\&TP) problem for one-way car-sharing services by taking into account the necessary practical requirements of vehicle relocation and personnel assignment. A mixed-integer nonlinear and nonconvex programming model is developed. Li et al. \cite{li2016adaptive} focus on the Share-a-Ride Problem (SARP) aiming at maximizing the profit of serving a set of passengers and parcels using a set of homogeneous vehicles. An  adaptive large neighborhood search heuristic algorithm is devised. Zhao et al. \cite{zhao2018integrated} devise an integrated framework to minimize the total cost, including the EV and staff investment, EV re-balancing and staff relocation costs. The model is reformulated and solved by Lagrangian relaxation approach. Boyacı et al. \cite{boyaci2015optimization} explore one-way vehicle-sharing systems that is taking vehicle relocation and electric vehicle charging requirements into consideration. A multi-objective optimization model is developed and solved by branch-and-bound. 

\par
For stochastic programming model, Brandstätter et al.\cite{brandstatter2017determining} solve strategic optimization problems of car-sharing systems that utilize electric cars by a two-stage stochastic programming model. Also, the heuristic algorithm is used to tackle large-scale instances. Biondi et al. \cite{biondi2016optimal} explore to optimize car-sharing system with uncertain demands from the perspective of queue theory. Fan et al. \cite{fan2004multi} consider the stochastic dynamic vehicle allocation problem (SDVAP), a multi-stage stochastic programming model is formulated to maximize profits and to manage fleets of vehicles in both time and space. Later, they develop a stochastic programming model to optimize strategic allocation of vehicles for one-way car-sharing systems under demand uncertainty
\cite{fan2014optimizing}. Cavagnini et al. \cite{cavagnini2018two} propose a bike-sharing system which composes one depot and multiple capacitated stations. 









==> 4-methodology.tex <==
\section{Methodology}



\begin{figure}[h]
    \centering
    \includegraphics[width = 13cm]{images/foo.eps}
    \caption{The framework of integration KDE and SP}
    \label{fig:1}
\end{figure}


\subsection{Kernel Density Estimation}
Kernel Density Estimation (KDE) is a non-parametric approach (also known as Parzen-Rosenblatt window method) to estimate the probability distribution function (PDF) of random variables. The significant of KDE is that it is capable of extracting any type of probability distributions.

\subsection{Stochastic Programming}
Stochastic Programming (SP) is a powerful modeling paradigm for decision making under uncertainty that aims to optimize the expected objective value across all the uncertainty realizations \cite{birge2011introduction}. The key idea of the SP approach is to model the randomness in uncertain parameters with probability distributions. The uncertainty described in SP is called scenarios. Most existing works related to SP is assumed that the probability distribution is known or estimated by parametric approaches. However, in the real applications, the probability distributions of data are not always ideal, therefore, we consider using non-parametric approaches such as the aforementioned KDE to derive the more appropriate probability distributions.



